Safe Platooning of Unmanned Aerial Vehicles via Reachability

Recently, there has been immense interest in using unmanned aerial vehicles (UAVs) for civilian operations such as package delivery, firefighting, and fast disaster response. As a result, UAV traffic management systems are needed to support potentially thousands of UAVs flying simultaneously in the airspace, in order to ensure their liveness and safety requirements are met. Hamilton-Jacobi (HJ) reachability is a powerful framework for providing conditions under which these requirements can be met, and for synthesizing the optimal controller for meeting them. However, due to the curse of dimensionality, HJ reachability is only tractable for a small number of vehicles if their set of maneuvers is unrestricted. In this paper, we define a platoon to be a group of UAVs in a single-file formation. We model each vehicle as a hybrid system with modes corresponding to its role in the platoon, and specify the set of allowed maneuvers in each mode to make the analysis tractable. We propose several liveness controllers based on HJ reachability, and wrap a safety controller, also based on HJ reachability, around the liveness controllers. For a single altitude range, our approach guarantees safety for one safety breach; in the unlikely event of multiple safety breaches, safety can be guaranteed over multiple altitude ranges. We demonstrate the satisfaction of liveness and safety requirements through simulations of three common scenarios.

==> analysis.tex <==
\section{Analysis}
Safety: 
\begin{itemize}
\item There always exists a safety control to keep the system safe for a prescribed time horizon despite the worst case disturbances 
\item Pairwise safety is translated into safety among all vehicles in the platoon \textcolor{blue}{thanks to linear chain and platoon assumptions. (Main proposition?)}
\item \textcolor{blue}{Safety with respect to intruder vehicles: under what exact conditions? What can we prove?}
\end{itemize}

